DORi: Discovering Object Relationship for Moment Localization of a Natural-Language Query in Video

This paper studies the task of temporal moment localization in a long untrimmed video using natural language query. Given a query sentence, the goal is to determine the start and end of the relevant segment within the video. Our key innovation is to learn a video feature embedding through a language-conditioned message-passing algorithm suitable for temporal moment localization which captures the relationships between humans, objects and activities in the video. These relationships are obtained by a spatial sub-graph that contextualizes the scene representation using detected objects and human features conditioned in the language query. Moreover, a temporal sub-graph captures the activities within the video through time. Our method is evaluated on three standard benchmark datasets, and we also introduce YouCookII as a new benchmark for this task. Experiments show our method outperforms state-of-the-art methods on these datasets, confirming the effectiveness of our approach.

==> conclusion.tex <==
\section{Conclusion}

We have presented a novel approach to temporal moment localization in video. Our approach consists of a spatial-temporal graph for capturing the relationships between detected humans, objects and activities over time. Conditioned on a natural language query, we proposed a message passing algorithm that propagates information across the graph to ultimately infer the arbitrarily long segment in the video most likely described by the query. Using our approach we are able to achieve state-of-the-art results on several benchmark datasets.

==> emnlp_review.tex <==
Review #1 

    What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?

        This paper proposes a new moment localization model which relies on a spatio-temporal graph representation of a video and language based message passing system. Video queries are represented as a graph with subject, verb, and object nodes. Messages are passed based on the language query. Next, a bidirection GRU is applied to spatial graphs to predict start and end points of moments. Overall, the results are good and some ablations are included.

        Strengths:

            Paper is clearly motivated and well written.

            Proposed model makes intuitive sense and leads to good results on some (but not all) datasets. Additionally, actions are represented by features from the I3D action recognition model and humans/objects are represented by RCNN features. The proposed graph representation is a nice way to integrate information across models pretrained for different tasks.

            Results included on many different datasets.

        Weaknesses:

            The the spatial loss comes from prior work, it would be helpful to include a short description.

            Model novelty: language conditioned graph networks have been used for other language and vision tasks. However, I think the domain here is different enough that there are enough difference in the model that it is fine.

            Though the model does improve across many tasks, there are some places where this model does not perform as well; in particular some of the ActivityNet metrics. It would be nice to see more insight about this. In particular, it seems to me that the model performs particularly well on small datasets. This could be because of the strong features.

            It could be helpful to see a few more ablations. In particular, one question I have is how important is it to have the action representation from I3D? Could this also be represented by something that looks more like RCNN (perhaps RCNN trained on single frame action prediction -- something like this: https://arxiv.org/pdf/1412.2604.pdf). Another question I have is how important the temporal graph is. One could imagine training a binary frame classifier on top of the frame representations (is this frame part of the moment or not).

            There are no failure modes discussed.

    Reasons to accept

        This is a well written paper with solid results and an interesting method. Though similar methods have been used for other language and vision tasks, I think the target task of moment localization is different enough from prior work and of enough interest to the EMNLP community that this paper will be beneficial for many conference goers. 

    Reasons to reject

        I think the only reason to reject is if there is a better paper and accepting this paper means another paper cannot be accepted. 

    Reproducibility:	4
    Overall Recommendation:	4
    Questions for the Author(s)

        See weaknesses above. In a rebuttal I would be most interested in understanding the performance on ActivityNet as well as learning about some qualitative failure cases. 

    Missing References

        n/a 

    Typos, Grammar, Style, and Presentation Improvements

        n/a 


Review #2

    What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?

        In this manuscript, the authors propose to predict the start and end of an event described in natural language via language-conditioned message-passing with graphs constructed from both the query (in natural language) and the video. The spatial sub-graph is constituted of three types of linguistic nodes: subject-verb relationship node SV, subject-object relation node SN, and verb-object relation node VN, as well as three types for video nodes in each frame of the video: human node H, object node O, and activity node A. Each type of node is encoded with a corresponding detection technique and neural encoding model. Message-passing is carried out on this graph among the nodes taking into account the query information. Then a temporal sub-graph works with the sequence of node representations and predicts the start and end of the event mentioned in the query. Strength: The problem is interesting, and the approach is technically sound, especially that the authors model the relationships among subject, object, and verb, which is different from other works that do not model these explicitly. The experimental results also show improvements, especially with a high IoU threshold.

        Weakness: However, the write up needs some effort to make the discussion clear enough for a publication. In the introduction, it would be better to have a clear clue leading to the challenge to be addressed, the approach to be used, and the contributions to be presented. The graph description is not very clear when it is firstly described at a high level. Figure 1 is there but not appropriately mentioned as the text reads. Supplemental material is somewhat helpful for understanding the approach, but it is not referenced in the text. It is hard to make a connection between the text and Figure 1. For the experiment, why is YouCookII taken out from the main comparison with baseline methods? Only TMLGA is compared on YouCookII, while LGVTI is a stronger baseline. A new model is somehow introduced, but neither the motivation nor result is well discussed.

        The authors need to make a significant improvement in presenting and in-depth discussing the motivation, approach, and results of this work. The technical contribution is interesting, but still limited but a stronger motivation and in-depth analysis will make this more interesting and insightful.

    Reasons to accept

        The problem is interesting, and the approach is technically sound, especially that the authors model the relationships among subject, object, and verb, which is different from other works. The experimental results also show improvement, especially with the high IoU threshold. 

    Reasons to reject

        The presentation is not well-prepared. The description is not always clear, and references to terms, notations, figures, and supplemental materials are not clear. There is no in-depth discussion about either the approach or the results. The technical contribution is limited/incremental. 

    Reproducibility:	3
    Overall Recommendation:	3


Review #3

    What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?

        This paper proposes an approach to localizing natural language queries in videos that encodes a spatio-temporal graph in order to make predictions. The approach is evaluated on 3 benchmark datasets.

        Strengths

        The approach appears to set a new SotA for certain metrics across the different datasets that are utilized. Additionally, modeling the input as a graph can have many potential benefits and this seems like a promising research direction.

        Weaknesses

        The method seems to be interesting but the writing and explanation of the method can be dense and confusing in many instances. For example, lines 323-334 discuss something about aggregating the text embeddings to "initialize three different heads of a multi-headed attention network..." However, not only is this section confusing and uses non-standard language, but the use of this aggregated vector appears no where else in the remainder of the paper. What exactly is this aggregated embedding and how is it used? Another example is that lines 411-417 attempt to describe what the "human" and "object" features are, but does so in a somewhat confusing way. Does the approach use Faster RCNN to detect objects in the image and the objects corresponding to humans or human attributes (e.g., arm, leg, ...) are assigned to the set H, and likewise for non-human objects and the set O? If so, it seems like simply stating that the approach takes the predicted labels for each object and categorizes them into human/non-human and assigns their corresponding features to human/non-human feature sets would suffice. Also, how are the linguistic nodes determined? Is dependency parsing used to determine the verb, subject, and object of the query? This is unclear and is not elaborated in the paper, but would appear to be important. Unfortunately, the diagram does not offer clarity either.

        The analysis portion of the paper leaves much to be desired. What happens if all the visual nodes are treated the same? Is there any insight as to why this model offers better performance at higher recall thresholds? Essentially, the experiments and ablation don't give much information towards what drives the performance, and instead discuss a few different hyperparameter choices (e.g., # of steps) and comparisons to other SotA models. There is nothing wrong with including these, but more analysis is important for others to build off this research.

        One last comment is that this approach seems to be tailored to cases where humans are the focal point of the activities, which may be fine as many activity recognition datasets tend to be "human-centric". I would be inclined to guess that if this method was evaluated on a set of videos that didn't have humans or where the query was not primarily about humans, then this method may perform worse. There is no analysis or discussion of this in the paper.

    Reasons to accept

        The paper presents an interesting, graph based approach towards phrase localization in videos. The experiments seem to show some promising results on this task. 

    Reasons to reject

        The paper is very confusing at times, many details/aspects of the approach are unclear, and there is little analysis of the approach. This could very well hinder the reproducibility of the method as well as the ability to build of this work. 

    Reproducibility:	2
    Overall Recommendation:	2.5
    Questions for the Author(s)

        Any clarification of the questions/concerns from the overall review above would be much appreciated.

        What exactly are the functions 'm' in equations 3,8,9?

        Can the authors explain, in their minds, the distinction between your method and that of Hu et al. (2019)? Conceptually, it appears that this method is almost the same with 2 caveats: 1) treating human and object nodes differently; 2) aggregating the action nodes through time with a GRU, in order to handle the temporal aspect. Does this seem accurate?

        What does the sentence on lines 428-431 mean? Do you have a citation or derivation of a "mean-field like approximation"?

        What is the "No LA" ablation in Table 2?

    Missing References

        The GRU cell is originally from Cho et al. (2014): https://www.aclweb.org/anthology/D14-1179/ 

    Typos, Grammar, Style, and Presentation Improvements

        Line 413: "huma‘n"

==> experiments.tex <==
\section{Experiments and Results}
\label{sec:experiments}

% In this section we give details about the experiments performed to test our proposed approach. We begin by describing the datasets used in our study, to later provide details about the training and evaluation procedures we followed. 

% \subsection{Datasets}

To evaluate our proposed approach we work with three widely utilized and challenging datasets, namely Charades-STA \cite{Gao_2017_ICCV}, ActivityNet Caption \cite{caba2015activitynet,Krishna_2017_ICCV} and TACoS \cite{tacos}. In addition to these, we also consider the YouCookII dataset \cite{ZhXuCoCVPR18,ZhLoCoBMVC18}. %This decision is motivated by its activity-centric nature as YoucookII is built upon instructional videos making it an excellent candidate to evaluate our proposals. %This is in contrast to other existing datasets that we do not consider here, specifically ActivityNet \cite{caba2015activitynet,Krishna_2017_ICCV}, which is annotated utilizing a descriptive approach that focuses on the video content rather than in the underlying action occurring. Below we proceed to give a quick description about each dataset.


\textbf{Charades-STA}: built upon the Charades dataset \cite{sigurdsson2016hollywood} which provides time-based annotations using a pre-defined set of activity classes, and general video descriptions. In Gao et al.\cite{Gao_2017_ICCV}, the sentences describing the video were semi-automatically decomposed into smaller chunks and aligned with the activity classes, which were later verified by human annotators. As a result of this process, the original class-based activity annotations are effectively associated to their natural language descriptions, totalling 13,898 pairs. We use the predefined train and test sets, containing 12,408 and 3,720 moment-query pairs respectively. Videos are 31 seconds long on average, with 2.4 moments on average, each being 8.2 seconds long on average. In our ablation studies we randomly split the train set in 80\% for training and 20\% for evaluation of the experiments.

\textbf{ActivityNet Captions}: Introduced by Krishna et al. \cite{Krishna_2017_ICCV}, this dataset which was originally constructed for dense video captioning, consists of 20k YouTube videos with an average length of 120 seconds. The videos contain 3.65 temporally localized time intervals and sentence descriptions on average, where the average length of the descriptions is 13.48 words. Following the previous methods, we report the performance  of  our algorithm on the combined two validation set.

\textbf{MPII TACoS}: built on top of the MPII Compositive dataset \cite{rohrbach2012script}, it consists of videos of cooking activities with detailed temporally-aligned text descriptions. There are 18,818 pairs of sentence and video clips in total  with the average video length being 5 minutes. A significant feature of this dataset is that due to the atomic nature of many of the descriptions ---e.g. ``takes out the knife`` and ``chops the onion''--- the associated video moments only span over a few seconds, with 8.4\% of them being less than 1.6 seconds long. This makes this dataset specially challenging for our task, as the relative brevity of the moments allows for a smaller margin of error. When it comes to splits, we use the same as in \cite{Gao_2017_ICCV}, consisting of 50\% for training, 25\% for validation and 25\% for testing.

% Why we decide to use youcookII? why this dataset is a good option to consider for the task? why haven't been use before?  
\textbf{YouCookII}: consists on 2,000 long untrimmed videos from 89 cooking recipes obtained from YouTube by Zhou et al. \cite{ZhXuCoCVPR18}. Each step for cooking these dishes was annotated with temporal boundaries and aligned with the corresponding section of the recipe. Recipes are written following the usual style of the domain \cite{linStyleVariationCooking,gerhardt2013culinary}, which includes very specific instruction-like statements with a wide degree of detail. The videos on this dataset are taped by individual persons at their houses while following the recipes using movable cameras. Similarly to TACoS, the average video length is 5.26 minutes. In terms of relevant moment segments, each video has 7.73 moments on average, with each segment being 19.63 seconds long on average. Videos have a minimum of 3 and a maximum of 16 moments. 

% \noindent
% \textbf{Charades-STA}: Collected from the Charades dataset \cite{sigurdsson2016hollywood} by adding sentences that describe actions in the videos, it consists on a total of 13,898 pairs of queries and temporal locations. We use the predefined train and test splits \cite{Gao_2017_ICCV}. Videos are 31 seconds long on average, with 2.4 moments on average, each being 8.2 seconds long on average.

% \noindent
% \textbf{ActivityNet Captions}: Introduced by \cite{Krishna_2017_ICCV} this dataset, which was originally constructed for dense video captioning, consists of 20k YouTube videos with an average length of 120 seconds. The videos contain 3.65 temporally sentence descriptions on average, where the average length of the descriptions is 13.48 words. Following previous work, we report the performance of our approach on the two existing validation sets combined \cite{munLocalGlobalVideoTextInteractions2020}.

% \noindent
% \textbf{MPII TACoS}: Built on top of the MPII Compositive dataset, it consists of videos of cooking activities with detailed temporally-aligned text descriptions. There are 18,818 pairs of sentence and video clips in total, with the average video length being 5 minutes. We use the same splits as \cite{Gao_2017_ICCV}, consisting of 50\% for training, 25\% for validation and 25\% for testing.

% \noindent
% \textbf{YouCookII}: consists on 2,000 long untrimmed videos from 89 cooking recipes obtained from YouTube by \cite{ZhXuCoCVPR18}. Each step for cooking these dishes was annotated with temporal boundaries and aligned with the corresponding section of the recipe. Similarly to TACoS, the average video length is 5.26 minutes. %In terms of relevant moment segments, each video has 7.73 moments on average, with each segment being 19.63 seconds long on average. Videos have a minimum of 3 and a maximum of 16 moments. 
% % % \smallskip
% % \noindent

\subsection{Implementation Details}

We first pre-process the videos by extracting features of size $1024$ using I3D with average pooling, taking as input the raw frames of dimension $256 \times 256$, at 25fps. We use the pre-trained model trained on Kinetics for TACoS, ActivityNet and YouCookII released by \cite{carreira2017quo}. For Charades-STA, we use the pre-trained model trained on Charades. We extract the top 15 object detections in terms of confidence for each of the keyframes using Faster-RCNN. %Note that this setup has been used by many previous methods~\cite{ghosh2019excl,rodriguez2019proposal,wangTemporallyGroundingLanguage2019,yuanSemanticConditionedDynamic2019,yuan2019semantic,zhang2018man}.

% Pre-processing for the natural language input in the case of Charades-STA is minimal, as we simply tokenize and keep all the words in the training data. In the case of ANEt-Cap, we pre-process the text with spacy\footnote{\url{https://spacy.io}} and replace all named entities as well as proper nouns with special markers. Finally, we truncate all sentences to a maximum length of 30 words and replace all tokens with frequency lower than 5 in the corpus with a special \textit{UNK} marker. The language encoder uses a hidden state of size $256$, without fine-tuning the pre-trained GloVe embeddings. 

All of our models are trained in an end-to-end fashion using ADAM \cite{kingma_adam} with a learning rate of $10^{-4}$ and weight decay $10^{-3}$. As mentioned earlier, our temporal graph is modeled using a two-layer BiGRU. We use a hidden size of $256$ and to prevent over-fitting we add a dropout of $0.5$ between the two layers.

\subsection{Evaluation}

We evaluate our model by two widely use metrics proposed by \cite{Gao_2017_ICCV}. The Recall at various thresholds of the temporal Intersection over Union ($R@\alpha$) measuring the percentage of predictions that have tIoU with ground truth larger than certain $\alpha$, and mean averaged tIoU (mIoU). We use three $\alpha$ threshold values $0.3$, $0.5$ and $0.7$.
% We evaluate our model by computing the temporal intersection over union (tIoU) at different thresholds, which we denote using the $\alpha$ parameter. In this setting, for a given value of $\alpha$, whenever a given predicted time window has a tIoU with the ground truth that is above the $\alpha$ threshold, we consider the output of the model as correct. 

% take a look at this for fixing the column width problem
% https://stackoverflow.com/questions/25688560/wrong-column-spacing-due-to-multicolumn-in-latex
\subsection{Ablation Study}

To show the effectiveness of our model we perform several ablation studies each aimed at assessing the contribution of a specific component. 

The ablative experiments in this section are based on a segment of the train split of the Charades-STA dataset. In addition to computing the tIoU for different thresholds, here we also report the mean tIoU (mIoU). As this metric provides a more comprehensive evaluation of the performance of our model, in fact we utilized mIoU to select the best model configuration for the rest of the experiments in this paper.

First, we study the impact of using different values of $N$, the number of iterations utilized in the message passing algorithm for our full model. Then, We choose the best $N$ to ablate the model and evaluate the role of each of the components. We start by removing the spatial loss in the training process, which encourages the model to focus on the features within the segment of interest. Then, we evaluate the importance of the human node by testing our model when assigning all the detected features to the object node. Finally, we test the contribution of the linguistic nodes by modifying our graph to only contain a single textual node which is connected to the rest of the graph in a way analogous to our full model. For details about these two last ablated models, please check C.1 and C.2 in the Supplementary Material. 

% To show the effectiveness of our model we perform several ablation studies each aimed at assessing the contribution of a specific component. First, we evaluate the role of the spatial loss that encourages the model to focus on the features within the segment of interest by training models without adding this term to the total loss. In addition to that, we evaluate the importance of modeling the subject who performs the actions in our spatio-temporal graph by testing models that lack these features. We also test the contribution of the linguistic nodes, modifying our graph to only contain a single textual node which is connected to the rest of the graph in a way analogous to our full model, please refer to the supplemental material. Finally, we also study the impact of using different values of $N$, the number of iterations utilized in the message passing algorithm for our full model.

% The ablative experiments in this section are based on a segment of the train split of the Charades-STA dataset. In addition to computing the tIoU for different thresholds, here we also report the mean tIoU (mIoU). As this metric provides a more comprehensive evaluation of the performance of our model, in fact we utilized mIoU to select the best model configuration for the rest of the experiments in this paper.

\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{c cccc c}
        \toprule
        \bf $N$ & R@0.3 & R@0.5 & R@0.7 & R@0.9 & mIoU \\
        \midrule
        0 & 47.46 & 22.88 & 14.38 & 6.00  & 33.67 \\
        1 & 73.21 & 55.32 & 36.02 & 11.48 & 52.11 \\
        2 & 79.01 & 67.16 & 48.71 & 17.97 & 59.30 \\
        3 & \textbf{79.25} & \textbf{68.41} & \textbf{50.56} & \textbf{19.14} & \textbf{60.29} \\
        4 & 70.99 & 60.31 & 44.16 & 17.32 & 54.01 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance when using a different number of iterations ($N$) for the message passing algorithm, on a subsection of the training split of Charades-STA.}
    \label{tab:res:n}
\end{table}

In terms of the role of the number of iterations of the message passing algorithm, as shown in Table \ref{tab:res:n}, we see that as $N$ increases performance increases as well, having a saturation point at $N=3$.

Table \ref{tab:res:ablations} summarizes the results of our ablation studies. As can be seen, the role of each one of our studied components is validated as the performance consistently drops for all the mIoU and most tIoU thresholds when ablating them. 

% In terms of the role of the number of iterations of the message passing algorithm, as shown in Table \ref{tab:res:n} we see that as $N$ increases performance increases as well. This tendency is revered ().

\subsection{Comparison with the state-of-the-art}

\begin{table}[t]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{ l cccc c}
        \toprule
        \bf Model & R@0.3 & R@0.5 & R@0.7 & R@0.9 & mIoU \\
        \midrule
        No $\mathcal{H}$ Node & 74.78 & 61.24 & 43.35 & 14.59 & 55.18 \\
        No LA & 76.79 & 66.32 & 49.92 & 20.87 & 58.93\\
        No $L_{\text{spatial}}$ & 76.79 & 66.60 & \textbf{52.54} & \textbf{23.57} & 59.95\\
        \midrule
        Full Model & \textbf{79.25} & \textbf{68.41} & 50.56 & 19.14 & \textbf{60.29}\\ \bottomrule
    \end{tabular}
    }
    \caption{Results of our ablation study on a section of the training split of Charades-STA.}
    \label{tab:res:ablations}
\end{table}

\begin{table*}[ht]
    \centering
    % \scriptsize %(asi)
    \scalebox{0.8}{
    \begin{tabular}{l c c c c c c c c c c c c}
        \toprule
        \multirow{2}{*}{\textbf{Method}} &\multicolumn{4}{c}{Charades-STA} & \multicolumn{4}{c}{ActivityNet} & \multicolumn{4}{c}{TACoS} \\
        & R@0.3 & R@0.5 & R@0.7 & mIoU & R@0.3 & R@0.5 & R@0.7 & mIoU & R@0.3 & R@0.5 & R@0.7 & mIoU\\ \midrule
        Random & - & 8.51 & 3.03 & - & 5.60 & 2.50 & 0.80 & & 1.81 & 0.83 & & - \\
        CTRL & - & 21.42 & 7.15 & - & 28.70 & 14.00 & - & 20.54 & 18.90 & 13.30 & - & - \\
        ABLR $\dag$ & - & 24.36 & 9.00 & - & 55.67 & 36.79 & - & 36.99 & 18.90 & 9.30 & - & - \\
        TripNet & 51.33 & 36.61 & 14.50 & - & 48.42 & 32.19 & 13.93 & - & 23.95 & 19.17 & 9.52 & - \\
        CBP & 50.19 & 36.80 & 18.87 & 35.74 & 54.30 & 35.76 & 17.80 & 36.85 & 27.31 & 24.79 & 19.10 & 21.59 \\
        MAN   & - & 46.53 & 22.72 & - & - & - & - & - & - & - & - & - \\
        EXCL  & 65.10 & 44.10 & 22.60 & - & - & - & - & - & \textbf{44.20} & 28.00 & 14.60 & - \\
        TMLGA & 67.53 & 52.02 & 33.74 & 48.22 & 51.28 & 33.04 & 19.26 & 37.78 & 24.54 & 21.65 & 16.46 & 22.06 \\ 
        LGVTI & \textbf{72.96} & 59.46 & 35.48 & 51.38 & \textbf{58.52} & \textbf{41.51} & 23.07 & 41.13 & - & - & - & - \\
        \midrule
        Ours & 72.72 & \textbf{59.65} & \textbf{40.56} & \textbf{53.28} & 57.89 & 41.49 & \textbf{26.41} & \textbf{42.78} & 31.80 & \textbf{28.69} & \textbf{24.91} & \textbf{26.42}\\ 
        \bottomrule
    \end{tabular}
    }
    \caption{Performance comparison of our approach with existing methods for different tIoU $\alpha$ levels. Values are reported on the validation split of Charades-STA and the ActivityNet Captions, and test splits for the TACoS datasets. $\dag$ Results for ABLR are as reported by \cite{sap2019}.}
    \label{tab:csta:res}
\end{table*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{imgs/visualization_sample_youcookii.pdf}
    \caption{Visualization of a success case of our method in the YouCookII dataset. The second row shows the observations associated to the Human node (green) and Object node (orange).}
    \label{fig:success:youcookii}
\end{figure*}

\begin{table}[t]
    \center
    \scalebox{0.9}{
    \begin{tabular}{l c c c c}
        \toprule
        \textbf{Method} & R@0.3 & R@0.5 & R@0.7 & mIoU \\
        \midrule
        Random & 4.84 & 1.72 & 0.60 & - \\ 
        TMLGA & 33.48 & 20.65 & 10.94 & 23.07 \\
        \midrule
        %  LaCoSTe {\tiny ECCV} & 42.70 & 29.04 & 16.29  \\  \hline
        Ours & \textbf{43.73} & \textbf{29.93} & \textbf{17.61} & \textbf{30.43} \\
        \bottomrule
        %  Ours & \textbf{68.87} & \textbf{54.38} & \textbf{36.99}  \\  \hline
    \end{tabular}
    }
    
    \caption{Performance on \textbf{YouCookII} for different tIoU $\alpha$ levels.}
    \label{tab:youcookii:res}
\end{table}

We compare the performance of our proposed approach on the datasets considered against several prior work. We consider a broad selection of models based on different approaches, specifically proposal-based techniques including CTRL \cite{Gao_2017_ICCV}, MAN \cite{zhang2018man} and CBP \cite{wang2019temporally}, as well as TripNet \cite{hahn2019tripping}, a method based on reinforcement learning. In addition to that, 
we also compare our approach to more recent methods that do not rely on proposals, including ABLR \cite{yuan2018find}, ExCL \cite{ghosh2019excl}, TMLGA \cite{rodriguez2019proposal} and LGVTI \cite{munLocalGlobalVideoTextInteractions2020}. Finally, we also consider a random baseline that simply selects an arbitrary video segment as the moment for each example. 

Table \ref{tab:csta:res} summarizes our results on the datasets Charades-STA, ActivityNet Captions and TACoS, while also comparing the obtained performance to relevant prior work. It is possible to see that our method is able to outperform previous work by a consistent margin, specially for the $\alpha=0.7$ band and also in terms of the mean tIoU (mIoU). Comparing results across these datasets, we also see that the performance of all models drops substantially on ActivityNet Captions and TACoS, compared to Charades-STA. We think this is mainly due to the nature of the dataset, which contains a considerable amount of video moments that only span a few seconds. 

% we note that  ExCL \cite{ghosh2019excl} experiments are not really comparable to the rest of the results on the table as they did not utilize all of evaluation data.

Finally, Table \ref{tab:youcookii:res} shows the performance of our model on the YouCookII dataset. To the best of our knowledge, since no previous work has been evaluated on this dataset we used the official implementation of TMLGA \cite{rodriguez2019proposal} released by its authors as an additional baseline. As can be seen, we are able to outperform both the random baseline and TMLGA by a large margin, specially on the lower $\alpha$ bands.  

\subsection{Qualitative results}

Figure \ref{fig:success:youcookii} presents a success case of our method on YouCookII dataset. The visualization is presenting a subsample of the key-frames inside of the prediction with their corresponding spatial observations, with green observations associated with the human node $\mathcal{H}$ and orange to the object node $\mathcal{O}$. Moreover, each visualization is presenting the ground-truth localization and predicted localization of the given query. As shown in Figure \ref{fig:success:youcookii}, given the query ``cover the dish with mashed potatoes'', our method could localize the moment at a tIoU of 98.88\%. The most relevant features extracted by Faster-RCNN to localize the query are {\em 'arm', 'bowl', 'cake', 'hand', 'kitchen', 'man', 'mug', 'spoon', 'stove', 'tray'}.

%In the case of Charades-STA, Fig. \ref{fig:success:charades}, given the query “a person is throwing the bag at the ligth switch” our method could localize the moment at a tIoU of 98.41\%. The most relevant features extracted by Faster RCNN for this query are {\em 'bag', 'light', 'person', 'wall'}. The full list of spatial features labels for each example can be find in the supplementary material. 
Additional qualitative examples of success and failure cases of our method are included in the section E of the Supplementary Material.



==> intro.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}

This paper studies the task of temporal moment localization in a long untrimmed video using natural language query.  Given a query sentence, the goal is to determine the start and end of the relevant segment within the video.
Our key innovation is to learn a video feature embedding through a language-conditioned message-passing algorithm suitable for temporal moment localization which captures the relationships between humans, objects and activities in the video. These relationships are obtained by a spatial subgraph that contextualized the scene representation using detected objects and human features. Moreover, a temporal sub-graph captures the activities within the video through time. Our method is evaluated on three standard benchmark datasets, and we also introduce YouCookII as a new benchmark for this task. Experiments show our method outperforms state-of-the-art methods on these datasets, confirming the effectiveness of our approach.  
\end{abstract}

% original version
% In this work we address the problem of temporal sentence localization in long untrimmed videos. Given a sentence and a video our task is to determine the starting and ending of the sentence in the video.
% Previous methods address the problem by learning a subspace to ranking the correlation between video's slices and language queries.
% In order to select the starting and ending time for a given text description on the corresponding video clip, we propose a novel guided attention method. Using the video and sentence representation we construct a temporal feature attention that is forced to attend intra features.
% Using recurrent network we predict start-end times. 
% We evaluate the proposed method on two public datasets Charades-STA and Activity Net Captions. Experimental results shows that our method outperform the state-of-the-art.

% More for abstract
% learning a subspace to ranking the correlation between video's slices and language queries . Using the video and sentence representation we construct a temporal feature attention that is forced to attend intra features
% Using recurrent network we predict start-end times. 
% as reflected in the low inter-annotator agreement 


\section{Introduction}

% Figure that summarizes the task and what we propose
Vision-and-language understanding is an important problem which has attracted increasing attention from both the computer vision and natural language processing communities over the past years. This research area includes tasks such as video captioning and video question answering.
% motivated by its vast potential applications. 
While promising results have been achieved on these tasks, a lot of work still needs to be done to help identify and trim informative video segments in longer videos, and align them with relevant textual descriptions. For this reason, tasks such as automatically recognizing \textit{when} an activity is happening in a video have recently become crucial for video analysis. 

\begin{figure}[t]
 \centering
 \includegraphics[width=0.5\textwidth]{imgs/IntroImage2.pdf}
 \caption{An illustration of temporal localization of a natural language query in an untrimmed video. Given a query and a video the task is to identify the temporal start and end of the sentence in the video.}
 \label{fig:example}
\end{figure}

As the amount of video data continues to grow, searching for specific visual events in large video collections has become increasingly relevant for search engines. This has helped draw increased attention to the task of activity detection in recent years. This is especially important considering that performing this task manually is laborious and error-prone, even for a small number of videos. In this sense, it is clear that search engines have to retrieve videos not only based on video metadata, but that they must also consider the video's content in order to accurately localize a given query. Applications in practical areas such as video surveillance and robotics~\cite{Liu_ICRA_2018} have also helped bring interest into this task. 

% Earlier work in this context has focused on {\em temporal action localization} \cite{richard2018neuralnetwork,lin_single_2017,escorcia_daps:_2016,Chao2018,GaoYSCN17,xu2019multilevel}, which attempts to localize interesting actions in a video from a predefined set of actions. As this constrains the search to a limited set of queries,  was proposed to address this issue. 
In relation to the aforementioned issue, in this paper we are specifically interested in the task of temporal sentence localization, where given an untrimmed video and a natural language query, the goal is to identify the start and end points of the video segment (i.e., moment) that best corresponds to the given query. This task can be seen as a generalization of temporal action localization task \cite{richard2018neuralnetwork,lin_single_2017,escorcia_daps:_2016,Chao2018,GaoYSCN17,xu2019multilevel}.% language~\cite{Gao_2017_ICCV,Hendricks_2017_ICCV}, which itself extends temporal action localization

%in the problem of natural language based queries, or temporal sentence localization in the video. Formally,
%Concretely, given a query the goal is to determine the start and end locations of the associated video segment in a long untrimmed video. 
%, as depicted in Figure \ref{fig:example}.
Many of the existing approaches to the localization problem in vision-and-language, either spatial or temporal, have focused on creating a good multi-modal embedding space and generating proposals based on the given query. 
%In these \textit{propose and rank} approaches, candidate regions are first generated by a separate method and then fed to a classifier to get the probabilities of containing target classes, effectively ranking them. %Most recently, approaches that do not rely on proposals to tackle this task have also been proposed. This mainly includes the work of Ghosh et al. \cite{ghosh2019excl} and Rodriquez et al. \cite{rodriguez2019proposal}. 
Most recently, approaches that do not rely on proposals to tackle this task have also been proposed, including the work of Ghosh et al. \cite{ghosh2019excl} and Rodriguez et al. \cite{rodriguez2019proposal}. Compared to proposal-based approaches, these techniques are more efficient and can handle the temporal relationship between activities better.

Evidence shows that solving grounded language tasks such as ours often requires reasoning about relationships between objects in the context of the task~\cite{huLanguageConditionedGraphNetworks2019}. For example, the work of \cite{sigurdsson_ICCV_2017} showed that the performance in action recognition tasks improves by a large margin if we have a perfect object recognition oracle. In our case, this evidence suggests that despite the success of proposal-free approaches, these techniques may be further improved by incorporating the information of the subjects and objects that appear in the video.

%will have limited power as long as they remain unable to incorporate a mechanism to capture and model the relationships between the subjects and objects that appear in the video. 

In light of this, in this paper we propose a mechanism to obtain contextualized activity representations based on a language-conditioned message passing algorithm. As activities are usually the result of the composition of several actions or interactions between a subject and objects \cite{jiang_IJMIR_2013}, our algorithm incorporates both spatial and temporal dependencies, modelling not only the relationship between subjects and objects in a scene but also how these change over time, to support the temporal moment localization task.\footnote{We will release features, pre-trained models and code upon acceptance.}
% In addition, our model also incorporates components that are known to be beneficial for the task \cite{ghosh2019excl,rodriguez2019proposal}.

%we tailor the activity feature representation (i3d) through a conditional languaged message passing algorithm to be good for temporal moment localization by understanding . This is captured by a spatial graph that contextualized the scene representation using the objects and human representation extracted by the object detector. Finally. the temporal graph capture the activities between the scenes during the time

We conduct experiments on four challenging datasets, Charades-STA \cite{Gao_2017_ICCV}, ActivityNet \cite{caba2015activitynet,Krishna_2017_ICCV}, TACoS \cite{tacos} and YouCookII \cite{ZhXuCoCVPR18,ZhLoCoBMVC18}, demonstrating the effectiveness of our proposed method and obtaining state-of-the-art performance. %PUNCHLINE AND CONTRIBUTIONS HERE.
Our results highlight the importance of our message-passing algorithm in modelling the relationship between human and object interaction to understand an activity, ultimately validating our proposed approach. 
To the best of our knowledge, our approach is the first to incorporate a language-conditioned message-passing algorithm to obtain contextualized activity representations using the objects and subjects. 

==> method.tex <==
\section{Graph Based Temporal Moment Localization}
\label{sec:method}

% Limitations/Comments
% --------------------

% 1.- We do not have have a way to know the gold standard objects in the query (or in the video?). Since the object detector we use in this work was not trained to detect objects conditioned on a given natural language input, but rather is only able to find "general" objects, the object representations we utilize in this work are () noisy. This is the main reason why we choose to work with a limited number of objects rather than with all the objects detected.
% 2.- Compared to other proposal-free approaches for our task, our main limitation is concerned with the length of the video, as our approach is computationally more expensive than these works. To alleviate this issue it is possible to utilize pooling techniques over the time to decrease the effective number of time-steps, at the possible cost of some overall performance degradation. This is proposed for future work.
% 3.- Arguably, our approach does not exactly perform message-passing as some nodes are grouped together before the message-passing step is performed. The main motivation to merge all the object nodes into a single representation is that capturing object-to-object relations is arguably less relevant for our task, where the main focus is the human action. This ultimately means that modeling subject-object relations is the key for (). Intuitively, our formulation can be also interpreted as way of modelling the relation between the subject and the expected objects in the scene.


%Graph networks are powerful models that can perform relational inference through message passing [4, 11, 21, 23, 38, 46]. The core idea is to enable communication between image regions to build contextualized representations of these regions. Graph networks have been successfully applied to various tasks, from object detection [26] and region classification [7] to human-object interaction [32] and activity recognition [14]. Besides, self-attention models [37] and non-local networks [40] can also be cast as graph networks in a general sense. 

In temporal moment localization, the objective is to find the location of a natural language query $Q$ in an untrimmed video $V$. The video consists of a sequence of frames $V=[ v_t \mid t = 1, \ldots, \ell ]$ and the query is a sequence of words $Q = [ w_j \mid j = 1, \ldots, m ]$ that describes a short moment in the video. We denote the starting and ending times of the moment described by query $Q$ as $t^s$ and $t^e$, respectively. 

We propose a model that explicitly captures the relationship between objects and humans, as well as the activities performed in a video, using a spatio-temporal graph. Concretely, we utilize a language-conditioned message passing algorithm, which allows us to obtain contextualized activity representations for better moment localization. Let $\mathcal{G} = (\mathcal{V}, \mathcal{E}_S \cup \mathcal{E}_T)$ represent our spatio-temporal graph, where $\mathcal{V}$, $\mathcal{E}_S$ and $\mathcal{E}_T$ are the set of nodes, spatial edges and temporal edges, respectively. 

We factorize our spatio-temporal graph into spatial and temporal sub-graphs, denoted by $\mathcal{G}_{S} = (\mathcal{V}, \mathcal{E}_S)$ and $\mathcal{G}_{T} = (\mathcal{V}, \mathcal{E}_T)$, respectively.

The spatial graph is designed to improve the \emph{activity representations} by exploiting the relationships between objects and humans in a given scene conditioned on the input query.
As we know \cite{sigurdsson2017actions}, actions and moments are characterized by complex interactions between humans as well as human-object interactions. Our spatial sub-graph is designed to specifically exploit these spatial relationships. It is iteratively applied through the video.

On the other hand, the temporal sub-graph is designed to model the relationships between the improved activity representations at different times to more efficiently localize the start and end point of the query in the video.

\subsection{Spatial graph} 

Consider the query presented in Figure \ref{fig:method:overview}, ``\textit{a person is throwing the bag at the light switch}''; it describes what action (\textit{verb}) is performed by a \textit{subject} and what \textit{objects} are involved in that action. Our spatial graph is designed to capture the relationships between these visual entities conditioned on the linguistic entities. As such, we decompose our graph into six semantically meaningful nodes, three for representing visual information and three for representing linguistic information. 

\subsubsection{Linguistic Nodes}

We create language nodes to capture essential information in the query related to the visual input: the \textit{subject-verb} relationship node $\mathcal{SV}$ (person-throwing), the \textit{subject-object} relation node $\mathcal{SN}$ (person-bag/light switch) and the \textit{verb-object} relation node $\mathcal{VN}$ (throwing-bag/light switch). 

% To obtain representations for each one of the linguistic nodes, we start by encoding the query using a function $F_Q: Q \mapsto \bold{h}$, which maps each word $w_j$ for $j = 1, \ldots, m$ in the query $Q$ to a semantic embedding vector $h_j \in \mathbb{R}^{d_w}$, where $d_w$ defines the hidden dimension of the word embedding. In this work we use GLoVe embeddings \cite{pennington_2014_EMNLP_glove} to obtain the vector representations for each word.

To obtain representations for each one of the linguistic nodes, we start by encoding each of the words $w_j$ for $j = 1, \ldots, m$ in the query $Q$ using a function $F_w: w \mapsto h$, which maps each word to a semantic embedding vector $h_j \in \mathbb{R}^{d_w}$, where $d_w$ defines the hidden dimension of the word embedding. Specifically, we use GLoVe embeddings \cite{pennington_2014_EMNLP_glove} to obtain the vector representations for each word.

% Later, these representations are aggregated into a fixed-length query vector $q$ which we use to initialize three different heads of a multi-head attention network \cite{vaswani2017attention}. Each head attends the encoded word vectors $h_j$ with $j = 1, \ldots, m$ and returns a re-weighted combination of them, aimed at understanding a specific relation between the visual nodes. our aggregation function is composed of a bi-directional GRU \cite{chung2014empirical} and mean pooling, allowing us to more accurately capture the global meaning of the input query by first contextualizing each word representation.

Later, these representations are aggregated into a fixed-length query vector $q$ which we use to initialize three different heads of a multi-head attention network \cite{vaswani2017attention}. Each head attends the encoded word vectors $h_j$ with $j = 1, \ldots, m$ and returns a re-weighted combination of them, aimed at understanding a specific relation between the visual nodes. Our aggregation function is composed of a bi-directional GRU \cite{chung2014empirical} and mean pooling, allowing us to more accurately capture the global meaning of the input query by first contextualizing each word representation.
%Therefore, our query function $F_Q$ is parameterized by both GLoVe embeddings and the GRU. 

% Then we create three different heads by using a linear projection of the query representation and for each of the word $w_j$ we generate an attention by:

% \begin{equation}
% \text{softmax}(QK^T)V
% \end{equation}

% Each of the linguistic nodes receives a high-dimensional representation of the natural language query $Q$. 
% the query node $\mathcal{Q}$ receives a high-dimensional representation (denoted by $q$) of the natural language query $Q$. 
% This high-dimensional representation is constructed using a function $F_Q: Q \mapsto q$ that first maps each word $w_j$ for $j = 1, \ldots, m$ in the query to a semantic embedding vector $h_j \in \mathbb{R}^{d_w}$, where $d_w$ defines the hidden dimension of the word embedding. Representations for each word are then aggregated using mean pooling to get a semantically rich representation of the whole query. %Concretely, we use mean pooling to obtain the final representation of the query.

% Although the query node is generic, in this work we use a bi-directional GRU \cite{chung2014empirical} on top of GLoVe word embeddings, which are pre-trained on a large collection of documents, for computing the $h_j$. Therefore, our query function $F_Q$ is parameterized by both GLoVe embedding and the GRU. 
% The query encoder aims at generating a semantically rich representation of the natural language query that is useful for localizing relevant moments in the video. We model our encoder as a function $F_S(S)$ that maps each word $s_j$ for $j = 1, \ldots, m$ to a semantic embedding vector $h_j \in \mathbb{R}^{d_s}$, where $d_s$ defines the hidden dimension of the obtained sentence representation. 


\subsubsection{Visual Nodes}

% Each of the semantically similar observations are associated with the same semantic node.
As mentioned above, our spatial graph contains three semantically meaningful nodes that represent visual information, specifically an activity node $\mathcal{A}$, a human node $\mathcal{H}$ and an object node $\mathcal{O}$. This setting allows us to share factors for semantically similar observations taken from the video \cite{jainStructuralRNNDeepLearning2016}, which provides several advantages. First, the model can deal with more observations of objects and humans without increasing the number of parameters that need to be learnt. Second, we alleviate the problem of having jittered object detections in videos, specially due to objects appearing and disappearing across frames.

To capture the relationships between activity, human and object observations, we densely connect these nodes within a single video frame. Such relationships are commonly parameterized by factor graphs that convey how a function over the graph factorizes into simpler functions~\cite{kschischang2001factor}. Similarly, we
learn a non-linear mapping function for each of the semantically alike observations that are associated with the same semantic node. In this sense, each semantic node, human $\mathcal{H}$, object $\mathcal{O}$ and activity $\mathcal{A}$, is considered to be a latent representation of the corresponding observation. Let us take as an example the case of the object node $\mathcal{O}$, where we observe a \textit{table} in the video, represented by a feature vector $x$, obtained directly from the object detector. In this case, we use a function $\Psi_{\scriptscriptstyle\mathcal{O}} \doteq \tanh ( W_{\scriptscriptsize\mathcal{O}} x + b_{\scriptscriptsize\mathcal{O}} )$. Similar mapping functions (with different parameters), namely $\Psi_{\scriptscriptstyle\mathcal{H}}$ and  $\Psi_{\scriptscriptstyle\mathcal{A}}$ are defined for the other semantic nodes.

\textbf{Activity node}: We use a video encoder that generates a video representation summarizing spatio-temporal patterns directly from the raw input frames. Concretely, let $F_V$ be our video encoding function that maps a video to a sequence of vectors $[ a_i \in \mathbb{R}^{d_v} \mid i = 1, \ldots, t]$.
These features capture high-level visual semantics in the video. 
Note that length of the video, $\ell = |V|$, and the number of output features, $t = |F_V(V)|$, are different due to temporal striding.
Specifically, in this work we model $F_V$ using I3D \cite{carreira2017quo}. This method inflates the 2D filters of a well-known convolutional neural network, e.g., Inception \cite{szegedy2015going,ioffe2015batch} or ResNet \cite{He_2016_CVPR} for image classification to obtain 3D filters. %However, I3D has not been tailored to solve our task. To tackle this problem we propose to make use of spatial information of objects and humans.

\textbf{Human and object nodes}: Activity representations are obtained using small clips of frames. This means that there may be a set of many frames from where to extract spatial information that is semantically relevant for each node.
Utilizing every frame is computationally expensive and given the piecewise smooth nature of video, this could also prove to be redundant. As such, in this work we propose to utilize key-frames associated to each activity representation to extract observations for human and object nodes. Since many frames in a video are blurry due to various reasons, e.g., the natural movement of the objects and the camera  motion, we select the sharpest key-frame in the subset of frames. Here we use the Laplace variance algorithm \cite{pech2000diatom}, which is a well-known approach for measuring the sharpness of an image.

While our method is agnostic to the choice of object detector, in this work we use Faster RCNN~\cite{ren_NIPS_2015_faster,anderson2018bottom} for the detection and spatial representation of the objects in all keyframes. Our Faster RCNN detector is trained on the Visual Genome \cite{krishnavisualgenome} dataset, which consists of 1,600 object categories. 
These categories are manually assigned to either the human and object nodes depending on the type of object. The human node receives the set of features $H = \{h_1,...,h_K\}$ corresponding to the categories huma`n body parts, clothes and subjects. 
% % Those human node specific features categories are denoted by $H = \{h_1,...,h_K\}$.
The object node receives the set of features that are not associated to human labels, as determined by our manual label categorization, such that $O = \{o_1,...,o_J\}$.
% The object node receives the set of features $O = \{o_1,...,o_J\}$, where the categories are not related to the human, therefore, have not been assigned to the human node.

% % For each activity representation, which is compose of a small subset of frames, we select a keyframe that is use to extract spatial information to improve the activity representation. We select the sharpest or less blurry image in the subset of frames using the Laplace variance algorithm \cite{pech2000diatom}. 

% % Each feature of I3D represents a small clip of the video, around 8 frames, for each of those clips we select a key frame which will be used to extract spatial information. Concretely, we select the sharpest or less blurry image in the clip using Laplace variance \cite{pech2000diatom}. 

% % Using Faster RCNN \cite{ren_NIPS_2015_faster} pre-trained in Visual Genome \cite{krishnavisualgenome} we extract spatial representation of {\em objects} and {\em humans} in the selected frames.
% % \vspace{-1mm}

\subsubsection{Language-conditioned message passing}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{imgs/messagepassing.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

We argue that the setting of the scene contains important clues to improve the representation of a given activity. Examples of these clues are human clothes, objects that are present in the scene as well as their appearance. To the best of our knowledge, previous work on moment localization has not utilized this information.%, which we believe is important for our task.
Therefore, we propose to obtain an activity representation suitable for the moment localization task, by capturing object, human and activity relationships. Concretely, we use a mean-field like approximation of the message passing algorithm to capture such relationships. The messages sent between nodes are conditioned on the natural language query. We propose to use this approximation instead of the standard message passing algorithm due to high demand on memory and compute, specially to process all the key-frames in a given video. The messages are iteratively sent a total of $N$ times, which is a hyperparameter of our model. In the equations below, index $n=1,...,N$ denotes the iteration step for each of the nodes. In the rest of this subsection, we drop the temporal index $i$ in the activity feature $a$ since the message passing is done for each of the activity features independently.

% First, we capture the relationship between the high-dimensional representation of the query $\mathcal{SN}, \mathcal{SV}$ and $\mathcal{VN}$with any observation of the nodes human $\mathcal{H}$, object $\mathcal{O}$ and activity $\mathcal{A}$, using a linear mapping function $f$ specific for each node.
First, we capture the relationship between the visual observations of the nodes human $\mathcal{H}$, object $\mathcal{O}$ and activity $\mathcal{A}$ with the corresponding language nodes $\mathcal{SN}, \mathcal{SV}$ and $\mathcal{VN}$ that connect the semantic meaning of the visual nodes, using a linear mapping function $f$ specific for each node.

For instance, in the case of the object observations, the mapping functions $f$ are 
{\fontsize{9}{12}
\begin{align*}
f_{\scriptscriptstyle\mathcal{SN,O}}(\mathcal{SN},o^{j,n}) &= W_{sno} [\mathcal{SN};o^{j,n}] + b_{sno}=\Phi_{\scriptscriptstyle\mathcal{SN,O}}^{j,n}  \text{ and}\\
f_{\scriptscriptstyle\mathcal{VN,O}}(\mathcal{VN},o^{j,n}) &= W_{vno} [\mathcal{VN};o^{j,n}] + b_{vno}=\Phi_{\scriptscriptstyle\mathcal{VN,O}}^{j,n} \text{ ,}
\end{align*}
}%
% where $j$ is the j-th object observation in the object node $\mathcal{O}$. Similarly, we have a specific mapping function {\fontsize{12}{12}$\Phi_{\scriptscriptstyle\mathcal{SV,A}}^{n}$,$\Phi_{\scriptscriptstyle\mathcal{VN,A}}^n$,$\Phi_{\scriptscriptstyle\mathcal{SN,A}}^{k,n}$, and $\Phi_{\scriptscriptstyle\mathcal{SV ,A}}^{k,n}$} for the activity and human observations, where $k$ is the k-th human observation.
where $j$ is the j-th object observation in the object node $\mathcal{O}$. Similarly, we have a specific mapping function {\fontsize{9}{12}$f_{\scriptscriptstyle\mathcal{SV,A}}(\mathcal{SV},a^{n}) = \Phi_{\scriptscriptstyle\mathcal{SV,A}}^{n}$, $f_{\scriptscriptstyle\mathcal{VN,A}}(\mathcal{VN},a^{n})=\Phi_{\scriptscriptstyle\mathcal{VN,A}}^n$, $f_{\scriptscriptstyle\mathcal{SN,H}}(\mathcal{SN},h^{k,n})=\Phi_{\scriptscriptstyle\mathcal{SN,A}}^{k,n}$, and $f_{\scriptscriptstyle\mathcal{SV,H}}(\mathcal{SV},h^{k,n})=\Phi_{\scriptscriptstyle\mathcal{SV ,A}}^{k,n}$} for the activity and human observations, where $k$ is the k-th human observation.

For clarity, we explain the message passing algorithm using again the object node as an example. The object node $\mathcal{O}$ receives messages from the human $\mathcal{H}$ and the activity $\mathcal{A}$ nodes. %this should be observation or latent representation but it makes difficult to follow
The message from the human node is constructed using a linear mapping function that receives as an input the concatenation of the object-query relationship $\Phi_{\scriptscriptstyle\mathcal{SN,O}}^{j,n}$ and the aggregation of all the human-query relationships $\sum_k \Phi_{\scriptscriptstyle\mathcal{SN,H}}^{k,n}$. A similar process is done for the message received from the activity observations, as can be seen in Equation \ref{object:message1}, below.
\begin{align}
    \Psi^{j,n}_{\scriptscriptstyle\mathcal{H,SN,O}} &= f_{\scriptscriptstyle\mathcal{H,SN,O}}(\Phi_{\scriptscriptstyle\mathcal{SN,O}}^{j,n},\textstyle \sum_{k=1}^K\Phi_{\scriptscriptstyle\mathcal{SN,H}}^{k,n}) \\
    \Psi^{j,n}_{\scriptscriptstyle\mathcal{A,VN,O}} &= f_{\scriptscriptstyle\mathcal{A,VN,O}}(\Phi_{\scriptscriptstyle\mathcal{VN,O}}^{j,n},\Phi_{\scriptscriptstyle\mathcal{VN,A}}^{n})
    % \Psi^{n}_{\scriptscriptstyle\mathcal{H,SV,A}} &= f_{\scriptscriptstyle\mathcal{H,SV,A}}(\Phi_{\scriptscriptstyle\mathcal{SV,A}}^{n},\textstyle \sum_{k=1}^K \Phi_{\scriptscriptstyle\mathcal{SV,H}}^{k,n}) \nonumber\\ 
    % \Psi^{n}_{\scriptscriptstyle\mathcal{O,VN,A}} &= f_{\scriptscriptstyle\mathcal{O,VN,A}}(\Phi_{\scriptscriptstyle\mathcal{VN,A}}^{n},\textstyle \sum_{j=1}^{J} \Phi_{\scriptscriptstyle\mathcal{VN,O}}^{j,n}) \nonumber\\
    % \Psi^{k,n}_{\scriptscriptstyle\mathcal{O,SN,H}} &= f_{\scriptscriptstyle\mathcal{O,SN,H}}(\Phi_{\scriptscriptstyle\mathcal{SN,H}}^{k,n},\textstyle \sum_{j=1}^{J} \Phi_{\scriptscriptstyle\mathcal{SN,O}}^{j,n}) \nonumber\\
    % \Psi^{k,n}_{\scriptscriptstyle\mathcal{A,SV,H}} &= f_{\scriptscriptstyle\mathcal{A,SV,H}}(\Phi_{\scriptscriptstyle\mathcal{SV,H}}^{k,n},\Phi_{\scriptscriptstyle\mathcal{SV,A}}^{n})
    % \Psi^{j,n}_{\scriptscriptstyle\mathcal{H,SN,O}} &= g_{\scriptscriptstyle\mathcal{H,SN,O}}(f_{\scriptscriptstyle\mathcal{SN,O}},\textstyle \sum_{k=1}^Kf_{\scriptscriptstyle\mathcal{SN,H}}) \\
    % \Psi^{j,n}_{\scriptscriptstyle\mathcal{A,VN,O}} &= g_{\scriptscriptstyle\mathcal{A,VN,O}}(f_{\scriptscriptstyle\mathcal{VN,O}},f_{\scriptscriptstyle\mathcal{VN,A}})
    % \Psi^{j,n}_{\scriptscriptstyle\mathcal{H,SN,O}} &= f_{\scriptscriptstyle\mathcal{H,SN,O}}(\Phi_{\scriptscriptstyle\mathcal{SN,O}},\textstyle \sum_{k=1}^K\Phi_{\scriptscriptstyle\mathcal{SN,H}}) \\
    % \Psi^{j,n}_{\scriptscriptstyle\mathcal{A,VN,O}} &= f_{\scriptscriptstyle\mathcal{A,VN,O}}(\Phi_{\scriptscriptstyle\mathcal{VN,O}},\Phi_{\scriptscriptstyle\mathcal{VN,A}})
    \label{object:message1}
\end{align}
\vspace{-0.5 em}
\vspace{-1em}
{\fontsize{10.85}{12}
    \begin{align}
        o^{j,n+1} &= \sigma(m_o(\Psi^{j,n}_{\scriptscriptstyle\mathcal{H,SN,O}} \odot \Psi^{j,n}_{\scriptscriptstyle\mathcal{A,VN,O}}) \odot o^{j,0})
        \label{object:message2}
    \end{align}
}
Finally, the new representation of the object observation is computed using Equation \ref{object:message2}, where $o^{j,0}$ is the initial object representation, $\sigma$ is an activation function, $\odot$ is the Hadamard product and $m_o$ is a linear function with a bias that constructs the message for the object $o^j$. A similar process is applied for each observation, as can be seen in Equations \ref{other:message1a} to \ref{other:message1b} below, where we create the message for each edge and Equations \ref{other:message2a} to \ref{other:message2b} and show how these messages are later used to contextualize the features. Note that the parameters learnt for each specific case are shared. For instance, parameters for $f_{\scriptscriptstyle\mathcal{A,SV,H}}$ and $f_{\scriptscriptstyle\mathcal{H,SV,A}}$ are the same.
\begin{align}
\Psi^{n}_{\scriptscriptstyle\mathcal{H,SV,A}} &= f_{\scriptscriptstyle\mathcal{H,SV,A}}(\Phi_{\scriptscriptstyle\mathcal{SV,A}}^{n},\textstyle \sum_{k=1}^K \Phi_{\scriptscriptstyle\mathcal{SV,H}}^{k,n}) 
\label{other:message1a}\\ 
\Psi^{n}_{\scriptscriptstyle\mathcal{O,VN,A}} &= f_{\scriptscriptstyle\mathcal{O,VN,A}}(\Phi_{\scriptscriptstyle\mathcal{VN,A}}^{n},\textstyle \sum_{j=1}^{J} \Phi_{\scriptscriptstyle\mathcal{VN,O}}^{j,n}) \\
\Psi^{k,n}_{\scriptscriptstyle\mathcal{O,SN,H}} &= f_{\scriptscriptstyle\mathcal{O,SN,H}}(\Phi_{\scriptscriptstyle\mathcal{SN,H}}^{k,n},\textstyle \sum_{j=1}^{J} \Phi_{\scriptscriptstyle\mathcal{SN,O}}^{j,n}) \\
\Psi^{k,n}_{\scriptscriptstyle\mathcal{A,SV,H}} &= f_{\scriptscriptstyle\mathcal{A,SV,H}}(\Phi_{\scriptscriptstyle\mathcal{SV,H}}^{k,n},\Phi_{\scriptscriptstyle\mathcal{SV,A}}^{n})
\label{other:message1b}
% \Psi^{n}_{\scriptscriptstyle\mathcal{H,SV,A}} &= f_{\scriptscriptstyle\mathcal{H,SV,A}}(\Phi_{\scriptscriptstyle\mathcal{SV,A}},\textstyle \sum_{k=1}^K \Phi_{\scriptscriptstyle\mathcal{SV,H}}) \nonumber\\ 
% \Psi^{n}_{\scriptscriptstyle\mathcal{O,VN,A}} &= f_{\scriptscriptstyle\mathcal{O,VN,A}}(\Phi_{\scriptscriptstyle\mathcal{VN,A}},\textstyle \sum_{j=1}^{J} \Phi_{\scriptscriptstyle\mathcal{VN,O}}) \nonumber\\
% \Psi^{k,n}_{\scriptscriptstyle\mathcal{O,SN,H}} &= f_{\scriptscriptstyle\mathcal{O,SN,H}}(\Phi_{\scriptscriptstyle\mathcal{SN,H}},\textstyle \sum_{j=1}^{J} \Phi_{\scriptscriptstyle\mathcal{SN,O}}) \nonumber\\
% \Psi^{k,n}_{\scriptscriptstyle\mathcal{A,SV,H}} &= f_{\scriptscriptstyle\mathcal{A,SV,H}}(\Phi_{\scriptscriptstyle\mathcal{SV,H}},\Phi_{\scriptscriptstyle\mathcal{SV,A}})
\end{align}
\vspace{-2.5em}
{\fontsize{10.25}{12}
\begin{align}
        % o^{j,n+1} &= \sigma(m_o(\Psi^{j,n}_{\scriptscriptstyle\mathcal{H,SN,O}} \odot \Psi^{j,n}_{\scriptscriptstyle\mathcal{A,VN,O}}) \odot o^{j,0})
        % \label{object:message2}\\
        a^{n+1} &= \sigma(m_a (\Psi^{n}_{\scriptscriptstyle\mathcal{H,SV,A}} \odot \Psi^{n}_{\scriptscriptstyle\mathcal{O,VN,A}}) \odot a^{0}) 
        \label{other:message2a}\\
        h^{k,n+1} &= \sigma(m_h (\Psi^{k,n}_{\scriptscriptstyle\mathcal{O,SN,H}} \odot \Psi^{k,n}_{\scriptscriptstyle\mathcal{A,SV,H}}) \odot h^{k,0}) 
        \label{other:message2b}
\end{align}
}

\subsection{Temporal graph}
The temporal graph is responsible for predicting the starting and ending points of the moment in the video. It uses the previously computed activity representations $a^{i,N} \text{ for } i=1, \ldots, t$ where $N$ is the final iteration in the message passing. 
The temporal graph is implemented using a 2-layer bi-directional GRU \cite{chung2014empirical} which receives as input the improved activity representation, and it is designed to contextualize the temporal relationship between the activity features. To obtain a probability distribution for the start and end predicted positions, we utilize two different fully connected layers to produce scores associated to the probabilities of each output of the GRU being the start/end of the location. Then, we take the softmax of these scores and thus obtain vectors $ \hat{\boldsymbol {\tau}}^s, \hat{\boldsymbol{\tau}}^e \in \mathbb{R}^{T}$ containing a categorical probability distribution. Even though we do not constrain the starting and ending points to follow the right order in time, this does not result in any difficulties in practice.

\subsection{Training}

Our method is trained end-to-end on a training set consisting of annotated tuples $(V, Q, t^s, t^e)$. Note that each video $V$ may include more than one moment and may therefore appear in multiple tuples. We treat each training sample independently. Given a new video and sentence tuple $(V_r, Q_r)$, our model predicts the most likely temporal localization of the moment described by $Q_r$ in terms of its start and end positions, $t_r^{s\star}$ and $t_{r}^{e\star}$, in the video. We use the Kullback-Leibler divergence and an spatial loss proposed by Rodriguez et al. \cite{rodriguez2019proposal}. We explain this in more detail in the supplemental material. 
% Need to explain the spacial loss and the use of soft labeling
Given the predicted/ground truth starting/ending  times of the moment, we use the following loss function during training:
\begin{equation}
    L_{\text{KL}} = \displaystyle D_{\text{KL}}(\hat{\boldsymbol{\tau}}^s \parallel \boldsymbol {\tau}^s) + \displaystyle D_{\text{KL}}(\hat{\boldsymbol {\tau}}^e \parallel \boldsymbol {\tau}^e)
    \label{eq:kl_div}
\end{equation}
where $D_{\text{KL}}$ is the Kullback-Leibler divergence. 
Moreover, inspired by Rodriguez et al. \cite{rodriguez2019proposal}, we use a spatial loss that aims to create activity features that are good at identifying where the action is occurring. This loss, equation \ref{eq:spatial}, receives as input $\textbf{y} = \text{softmax}(g (\textbf{a}))$ where $\textbf{a}$ is the matrix that results by concatenating the improved activity representations over time, and $g$ is a linear mapping that gives us a score for each activity representation. We apply a softmax function over these and our loss penalizes if this normalized score is large for those features associated to positions that lie outside the temporal location of the query.

% Our method is trained end-to-end on a training set consisting of annotated tuples $(V, Q, t^s, t^e)$. %Note that each video $V$ may include more than one moment and may therefore appear in multiple tuples. We treat each training sample independently.
% Given a new video and sentence tuple $(V_r, Q_r)$, our model predicts the most likely temporal localization of the moment described by $Q_r$ in terms of its start and end positions, $t_r^{s\star}$ and $t_{r}^{e\star}$, in the video. We use the Kullback-Leibler divergence and an spatial loss proposed by \citet{rodriguez2019proposal}. More details in the Supplementary Material. 
% Need to explain the spacial loss and the use of soft labeling
% Given the predicted/ground truth starting/ending  times of the moment, we use the following loss function during training:
% \begin{equation}
%     L_{\text{KL}} = \displaystyle D_{\text{KL}}(\hat{\boldsymbol{\tau}}^s \parallel \boldsymbol {\tau}^s) + \displaystyle D_{\text{KL}}(\hat{\boldsymbol {\tau}}^e \parallel \boldsymbol {\tau}^e)
%     \label{eq:kl_div}
% \end{equation}
% where $D_{\text{KL}}$ is the Kullback-Leibler divergence. 
% Moreover, inspired by Rodriguez et al. \cite{rodriguez2019proposal}, we use a spatial loss that aims to create activity features that are good at identifying where the action is occurring. This loss, equation \ref{eq:spatial}, receives as input $\textbf{y} = \text{softmax}(g (\textbf{a}))$ where $\textbf{a}$ is the matrix that results by concatenating the improved activity representations over time, and $g$ is a linear mapping that gives us a score for each activity representation. We apply a softmax function over these and our loss penalizes if this normalized score is large for those features associated to positions that lie outside the temporal location of the query. %and forced the features to 
% \vspace{-1mm}
% \begin{equation}
%     L_{\text{spatial}} = - \sum_{i=1}^t (1- \delta_{\tau^s \leq i \leq \tau^e}) \log(1-y^i) %\frac{1}{B} \sum_{i=1}^B 
%     \label{eq:spatial}
% \end{equation}
% where $\delta$ is the Kronecker delta.
% The final loss for training our method is the sum of the two individual losses defined previously setting $\mathcal{L} =    L_{\text{KL}} + L_{\text{spatial}}$. 
% During inference, we predict the starting and ending positions using the most likely locations given by the estimated distributions, using $\hat{\tau}^s = \text{argmax}(\hat{\boldsymbol{\tau}}^s)$ and $\hat{\tau}^e = \text{argmax}(\hat{\boldsymbol{\tau}}^e)$. Since values correspond to positions in the feature domain of the video, so we convert them back to time positions.






==> relatedwork.tex <==
\section{Related Work}

% \subsection{Temporal action localization}

Our work is related to the task of temporal action localization, which aims to solve the problem of recognizing and determining temporal boundaries of action instances in videos. There is extensive previous work on this task, ranging from models that train existing video feature extractors with a localization loss \cite{Shou_2016_CVPR}, to systems that generally rely on temporal action proposal, as well as more sophisticated models that perform contextual modelling, capturing objects and their interactions \cite{guAVAVideoDataset2018,girdharVideoActionTransformer2019}.
%After the introduction of the AVA dataset \cite{guAVAVideoDataset2018}, which contains clips labeled with people and their actions, various proposals have attempted to perform contextual modelling, i.e. capturing objects and object interactions for action localization. This is the case of Girdhar et al. \cite{girdharVideoActionTransformer2019}, who recently proposed a Transformer-based model which uses its attention mechanism learns to emphasize hands and faces, which are often crucial to discriminate an action.


%In all cases, methods are often tested on the MPII-Cooking dataset \cite{rohrbach_dataset_2015} or on THUMOS \cite{idrees_thumos_2017}. In order to model the temporal nature of the task, these works have generally relied on time-sensitive architectures such as LSTMs \cite{ma_learning_2016,singh_multi-stream_2016,escorcia_daps:_2016} or temporal convolutions \cite{simonyan2014two,lin_single_2017}. 

%Since activities (in the wild) consist of a diverse combination of actors, actions and objects over various periods of time, earlier work focused on classification of video clips that contained a single activity, i.e., where the videos were trimmed. 
%More recently there has also been significant work in localizing activities in longer, untrimmed videos. 

%On the other hand, Ma et al.  used a temporal LSTM to generate frame-wise prediction scores and then merged the detection intervals based on the predictions. Singh et al.  extended the two-stream framework with person detection and bi-directional LSTMs and achieved state-of-the-art performance on the MPII-Cooking dataset . 
%Escorcia et al. \cite{escorcia_daps:_2016} took a different approach and introduced an algorithm for generating temporal action proposals from long videos, which are used to retrieve temporal segments that are likely to contain actions. 
%Lin et al. \cite{lin_single_2017} proposed an approach based on 1D temporal convolutional layers to skip the proposal generation step via directly detecting action instances in untrimmed video, obtaining excellent results on the THUMOS \cite{idrees_thumos_2017} and and MEXaction2 \cite{mexaction} datasets. 

% \subsection{Temporal language-driven moment localization}

%As it is non-trivial to design a label space which has enough coverage for such activities without losing useful details in users' queries this approach makes it difficult to cover complex activity queries. 
% Later, extended this work to leverage activity classifiers to encode visual concepts, while \cite{} used memory attention models when matching each proposal to the input query. 
Since action localization is restricted to a pre-defined list of options, Gao et al. \cite{Gao_2017_ICCV} and Hendricks et al. \cite{Hendricks_2017_ICCV} introduced a variation of the task called language-driven temporal moment localization, where the goal is to determine the start and end time of the temporal video segment that best corresponds to a given natural language query. Early approaches for this task, including Liu et al. \cite{liu2018attentive} and Ge et al. \cite{ge2019mac}, were mainly based on generating proposals or candidate clips which could later be ranked. More recently Chen et al. \cite{chen-etal-2018-temporally}, Chen and Jiang \cite{sap2019}, and Xu et al. \cite{xu2019multilevel}, have worked on reducing the number of proposals by producing query-guided or query-dependent approaches.

%Essentially, this means to use natural language queries to localize activities in untrimmed videos. While the language-based setting allows for having an open set of activities, it also corresponds to a more natural query specification, as it directly includes objects and their properties as well as relations between the involved entities. 

%On the other hand, Chen et al. \cite{sap2019} focused on the proposal generation step, integrating the semantic information of the natural language query into the proposal generation process to get discriminative activity proposals.

%Chen et al. \cite{chen-etal-2018-temporally} propose to capture frame-by-word interactions between video and language and then score a set of temporal candidates at multiple scales to localize the video segment that corresponds to the query. Similarly, Xu et al. \cite{xu2019multilevel} propose a multilevel model to tightly integrate language and vision features and then use a fine-grained similarity measure for query-proposal matching.

%Hendricks et al. \cite{Hendricks_2017_ICCV}, proposed to learn a shared embedding for both video temporal context features and natural language queries suitable for matching candidate video clips and language queries. They later further improved this approach by modelling the video context as a latent variable to reason about the temporal relationships \cite{Hendricks_2018_EMNLP}. 

%\cite{yuan2018find,ghosh2019excl,chenrethinking,rodriguez2019proposal,wangTemporallyGroundingLanguage2019,yuanSemanticConditionedDynamic2019,luDEBUGDenseBottomUp2019}
Despite their ability to provide coarse control over the video snippets, proposal-based methods suffer from the computationally expensive candidate proposal matching, which has led to the development of methods that can directly output the temporal coordinates of the segment. In this context, Yuan et al. \cite{yuan2018find} first proposed to use a co-attention-based model, and soon after Ghosh et al.\cite{ghosh2019excl} focused directly on predicting the start and end frames using regressions. More recently Rodriguez et al. \cite{rodriguez2019proposal} used dynamic filters and modeled label uncertainty to further improve performance, while \cite{munLocalGlobalVideoTextInteractions2020, zengDenseRegressionNetwork2020} proposed more sophisticated modality matching strategies. Compared to these works, although our approach is also proposal-free, we differ in the sense that we aim at incorporating specific spatial information that is useful for the localization problem. 

% The proposed method effec-
% tively predicts the target time interval by exploiting contex-
% tual information from local to global
% Local-{{Global Video}}-{{Text Interactions}} for {{Temporal Grounding}}},

%Dense {{Regression Network}} for {{Video Grounding}}},
  

% Even if the proposals are generated aligned with language semantics instead of fetching video clips independently, they still depend on ranking a fixed number of temporal candidates in each video, leading to inefficiencies. In light of this, some models have resorted to reinforcement learning to dynamically observe a sequence of video frames conditioned on the given language query \cite{wang2019language} to learn how to skip around the video \cite{hahn2019tripping}.% therefore being able to more easily localize relevant clips in long videos.

%However, for temporal localization of activities, it is unclear what a proper visual model to extract visual features for retrieval is, and how to achieve high precision of predicted start/end time. Although one could densely sample sliding windows at different scales, doing so is not only computationally expensive but also makes the alignment task more challenging, as the search space increases. An alternative to dense sampling is to adjust the temporal boundaries of proposals by learning regression parameters; such an approach has been successful for object localization, as in [23]. 

% Concretely, Wang et altrain a recurrent neural network for language-driven temporal activity localization using this approach, while also utilizing Faster R-CNN~\cite{ren_NIPS_2015_faster} trained on the Visual Genome dataset~\cite{krishnavisualgenome} to obtain regional visual features and incorporate more semantic concepts to the model. 

% Rethinking bottom-up framework for query based video localization AAAI20 \cite{chenrethinking}
% Temporally grounding language queries in videos by contextual boundary-aware prediction. AAAI (2020) 

% \cite{wangTemporallyGroundingLanguage2019}

% Semantic  conditioned  dynamic modulation  for  temporal  sentence  grounding  in  videos. NeurIPS(2019)
%\cite{yuanSemanticConditionedDynamic2019}

%DEBUG: A Dense Bottom-Up Grounding Approach for Natural Language Video Localization
%\cite{luDEBUGDenseBottomUp2019}

%\subsection{Context modelling in action understanding}

% start with papers that use graph for our task
% then talk about papers that use graphs for other things

% - Difference with structured RNN: their graph is not conditioned on the language.
Our work is also related to context modeling in action recognition. In this context, structural-RNN \cite{jainStructuralRNNDeepLearning2016} models a spatio-temporal graph using an RNN mixture that is differentiable, with applications on human motion modelling and human activity detection. While we build on top of a concept similar to this, we inject the language component into the spatio-temporal graph and focus on language-conditioned temporal moment localization.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{imgs/DORI_method.pdf}%
    \caption{For each activity feature $a_i$, we create a Spatial graph to find the relationship between object and human nodes conditioned in the query, and thus improve the activity representation to be used by the Temporal graph.}
    \label{fig:method:overview}
\end{figure*}
% Difference with "Language-conditioned graph": it does not include time and  the message passing is different since they focus on edges. Instead, our approach is node-based as we assume that the connections between different kinds of nodes have the same edge weights.
Context modeling has also been recently utilized in other computer vision tasks, such as referring expression comprehension \cite{yuMAttNetModularAttention2018} and VQA \cite{huLanguageConditionedGraphNetworks2019}. In the latter, the authors proposed a Language-Conditioned Graph Network (LCGN) where each node represents an object and is described by a context-aware representation from related objects through iterative message passing conditioned on the textual input. Our work is fundamentally different from this as our task requires us to model the temporal component on our graph. On the other hand, meanwhile LCGN emphasizes the role of edge representations in the graph, our approach is node-centric as connections between two given node types share the same edges.

Furthermore Zeng et al. \cite{zengGraphConvolutionalNetworks2019} used graph convolutions to obtain contextualized representations for action localization, while Zhang et al. \cite{zhang2018man} utilized a graph-structured network to model temporal relationships among different moments and thus obtain contextualized moment representations. Their approach is different from ours as they rely on proposals to perform the task. More recent approaches, such as SLTFNet \cite{jiang_sltfnet_2019}, rely on attention instead of message passing to deal with the spatio-temporal nature of the moment localization task. 

%Specifically, they use graphs to address semantic and structural misalignment problems that previous proposal-based methods had. 
%Their approach can be seen as an extension of \cite{yuMAttNetModularAttention2018} with the attention components capturing the interactions between objects for a given frame, and the relation to keywords in the query to each frame.

%As an action consists of multiple proposals in a video, they model proposal-to-proposal relations using GCNs to construct an action proposal graph and obtain contextualized representations for improving performance.

Finally, Zhang et al. \cite{zhangWhereDoesIt2020} have recently proposed a novel task which requires not only to perform temporal language-driven moment localization, but also to spatially locate the objects mentioned in the query. Their approach is similar to ours in the sense that it also utilizes a spatio-temporal graph. However, the textual clues are incorporated after the graph construction rather than being an explicit part of it.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In ECCV'17 two papers \textit{localizing moments with natural language} \cite{Hendricks_2017_ICCV} and \textit{temporal activity localization via language query} \cite{Gao_2017_ICCV} from different groups introduced a new problem. Temporally localize an activity in a video using natural language descriptions.

% Hendricks et. al. \cite{Hendricks_2017_ICCV} {\tiny[\textbf{Berkeley, Adobe}]} method learns to match natural language with intervals of a video. They learned a shared embedding space for video and language features. Video features are constructed using VGG16 for each frame (RGB and Optical Flow), then mean-pooling all the frames features in a global (all frames) and local manner. Finally, global and local video representation are concatenated. For the language modality, they pass the corresponding sentence through an LSTM. Last output of the LSTM is fed to an FC layer to get the sentence representation. 


% These two pieces of work naturally evolve in \cite{Hendricks_2018_EMNLP} and \cite{Ge_2019_WACV} respectively. Hendricks et. al. EMNLP'18 \cite{Hendricks_2018_EMNLP} exploits the temporal reference in a sentence. For instances, queries like \textit{the girl bends down} require understanding object and action, but do not require reasoning about different video moments. In queries like \textit{the little girl talks after bending down} it is necessary a temporal relationship reasoning about the different actions one happens after the other. They also create a dataset for this problem. In the case of \cite{Ge_2019_WACV} they just add the actionness score to the pipeline.

% % In other works: 

% Zhang et. al. CVPR'19 \cite{Zhang_2019_CVPR} found similar challenges with temporal semantics. They define two types of problems \textit{semantic misalignment} and \textit{structural misalignment}. First scenario, where a simple number will result in searching through the whole video and making that a sliding window approach would fail: For instance, a query like \textit{A child touches the ground the second time}. The second scenario, when the sentence is described backwards, such as \textit{Child is running away after is closest to the camera}. They propose to made use an iterative graph adjustment network IGAN to understand the relationship between actions.

% Chen S. et. al. AAAI'19 \cite{ChenS_2019_AAAI} and Chen J. et. al. AAAI'19 \cite{ChenJ_2019_AAAI} focus on efficiency of the algorithms proposed by Hendricks and Gao. Focusing on the proposal generation step, since Hendricks \cite{Hendricks_2017_ICCV} made use of an exhaustive enumeration of possible temporal regions and Gao \cite{Gao_2017_ICCV} used a naive sliding window to feed their methods, both are very inefficient. \cite{ChenS_2019_AAAI} propose a semantic activity proposal. Proposal are generated grouping frames that match with high visual-semantic correlation score.

% Similarly, Xu et. al. AAAI'19 \cite{XuH_2018_AAAI2} method generate proposals incorporating semantic in that stage, eliminating unlikely clips and thus speed up processing. Moreover, They learn a fine-grained similarity metric for retrieval, they used visual features to modulate the processing of query sentences at the word level in a recurrent neural network scheme. Notice that they are the first using \textbf{ANet-Caption} dataset \cite{Krishna_2017_ICCV} for moment retrieval and to the best of my knowledge the only one.

% It is interesting and challenging to see that are a lot of interest about this problem AAAI'19 \cite{ChenS_2019_AAAI, ChenJ_2019_AAAI, XuH_2018_AAAI2} and WACV'19 \cite{Ge_2019_WACV}. I believe mainly because we are generalizing the problem of activity localization/detection compare with the previous approach without natural language.


